3D Point Cloud Denoising using Graph Laplacian Regularization of a Low Dimensional Manifold Model

3D point cloud - a new signal representation of volumetric objects - is a discrete collection of triples marking exterior object surface locations in 3D space. Conventional imperfect acquisition processes of 3D point cloud - e.g., stereo-matching from multiple viewpoint images or depth data acquired directly from active light sensors - imply non-negligible noise in the data. In this paper, we adopt a previously proposed low-dimensional manifold model for the surface patches in the point cloud and seek self-similar patches to denoise them simultaneously using the patch manifold prior. Due to discrete observations of the patches on the manifold, we approximate the manifold dimension computation defined in the continuous domain with a patch-based graph Laplacian regularizer and propose a new discrete patch distance measure to quantify the similarity between two same-sized surface patches for graph construction that is robust to noise. We show that our graph Laplacian regularizer has a natural graph spectral interpretation, and has desirable numerical stability properties via eigenanalysis. Extensive simulation results show that our proposed denoising scheme can outperform state-of-the-art methods in objective metrics and can better preserve visually salient structural features like edges.

==> preliminary.tex <==
\subsection{Calculation of Manifold Dimension}
%In \cite{osher2017low}, the image is decomposed into overlapping patches, where each patch is of size $d$. The basic assumption is that these patches sample a low dimensional manifold $\mathcal{M}$ embedded in $\mathbb{R}^d$, which is called the patch manifold associated with the image.

Consider a smooth manifold $\mathcal{M}$ embedded in $\mathbb{R}^d$, and let $\alpha_i$, where $i=1,\dots,d$, be the coordinate functions on $\mathcal{M}$, \textit{i.e.},
\begin{equation}
\alpha_i(\mathbf{x}) = x_i, \forall \mathbf{x}=[x_1,\dots,x_d]^{\top} \in \mathcal{M}. 
\end{equation}
Here $\mathbf{x} \subset \mathbb{R}^d$ is a sample on $\mathcal{M}$. As proved in \cite{osher2017low}, the dimension of $\mathcal{M}$ at $\mathbf{x}$ can be calculated as,
\begin{equation}
\text{dim}(\mathcal{M})(\mathbf{x}) = \sum_{i=1}^{d} ||\nabla_{\mathcal{M}} \alpha_i(\mathbf{x})||^2,
\end{equation}
where $\nabla_{\mathcal{M}} \alpha_i(\mathbf{x})$ denotes the gradient of the function $\alpha_i$ on $\mathcal{M}$ at $\mathbf{x}$.
Then the integration of $\text{dim}(\mathcal{M})(\mathbf{x})$ over $\mathcal{M}$ is used as the regularization term in inverse image problems \cite{osher2017low}, given as,
\begin{equation}
\int_{\mathcal{M}} \text{dim}(\mathcal{M})(\mathbf{x}) d \mathbf{x} = \sum_{i=1}^{d} \int_{\mathcal{M}} ||\nabla_{\mathcal{M}} \alpha_i(\mathbf{x})||^2 d \mathbf{x}.
\end{equation}
%Notice that the analytical form of $\mathcal{M}$ is not known, and only a set of unstructured samples on $\mathcal{M}$ is given, making it difficult to compute the regularization term. In this case, a graph Laplacian is usually used to approximate the regularization in order to solve the optimization on the unstructured samples \cite{pang2017graph}.

\subsection{Graph Laplacian Regularization and its Continuous Limit}
\subsubsection{Constructing Graph on a Manifold}
Here we describe the construction of a discrete graph $\mathcal{G}$ where its vertices $\mathcal{P} = \{\mathbf{p}_j\}_{j=1}^M$ lie on a smooth manifold $\mathcal{M}$ embedded in $\mathbb{R}^d$, \textit{i.e.}, $\mathbf{p}_j \in \mathcal{M} \subset \mathbb{R}^d$.
Let $\mathcal{E}$ denote the edge set, where the edge between $i$-th and $j$-th vertices is weighted as,
\begin{equation}
w_{ij} = (\rho_i \rho_j)^{-1/2} \psi(d_{ij}).
\end{equation}
The kernel $\psi(\cdot)$ is a thresholded Gaussian function
$$\psi(d_{ij})=
\begin{cases}
\exp(-\frac{d_{ij}^2}{2\epsilon^2}) & \mathrm{if} d_{ij}<r \\
0& \text{otherwise},
\end{cases}$$
and $d_{ij}$ is the Euclidean distance between the two vertices $\mathbf{p}_i$ and $\mathbf{p}_j$,
\begin{equation}
d_{ij} = ||\mathbf{p}_i - \mathbf{p}_j||_2^2.
\end{equation}
The term $(\rho_i \rho_j)^{-1/2}$ is the normalization term, where $\rho_i = \Sigma_{j=1}^M \psi(d_{ij})$ is the degree of $\mathbf{p}_i$ before normalization. 
The graph constructed in these settings is an $r$-neighborhood graph, \textit{i.e.}, no edge has a distance greater than $r$. Here $r = \epsilon C_r$, and $C_r$ is a constant.

\subsubsection{Graph Laplacian Regularizer}
With the edge weights defined above, we have the symmetric adjacency matrix $\mathbf{A} \in \mathbb{R}^{M \times M}$, with the $(i,j)$-th entry given by $w_{ij}$. $\mathbf{D}$ denotes the diagonal degree matrix, where entry $\mathbb{D}(i,i) = \Sigma_j w_{i,j}$. The combinatorial graph Laplacian matrix is $\mathbf{L} = \mathbf{D} - \mathbf{A}$ \cite{shuman13}. 

For a smooth function $f$ defined on $\mathcal{M}$, \textit{i.e.}, $f \in C_c^{\infty}(\mathcal{M})$, sampling $f$ at positions of $\mathcal{P}$ leads to its discretized version, $\mathbf{f} = [f(\mathbf{p}_1), \dots, f(\mathbf{p}_M)]^{\top}$. The graph Laplacian $\mathbf{L}$ induces the regularizer $S_{\mathbf{L}}(\mathbf{f}) = \mathbf{f}^{\top} \mathbf{L} \mathbf{f}$. It can be shown that
\begin{equation}
S_{\mathbf{L}}(\mathbf{f}) = \mathbf{f}^{\top} \mathbf{L} \mathbf{f} = \Sigma_{(i,j)\in \mathcal{E}} w_{ij} (f(\mathbf{p}_i) - f(\mathbf{p}_j))^2.
\end{equation}

\subsubsection{Convergence of Graph Laplacian Regularizer}
According to the convergence proof in \cite{hein2007manifold}, 
\begin{equation}
\underset{M \rightarrow \infty, \epsilon \rightarrow 0} {\lim} \mathbf{f}^{\top} \mathbf{L} \mathbf{f} \sim  \int_{\mathcal{M}} ||\nabla_{\mathcal{M}} f(\mathbf{x})||_2^2 h(\mathbf{x}) d \mathbf{x},
\end{equation}
where $\sim$ means there exists a constant depending on $C_r$ and $\epsilon$, such that the equality holds.
$h(\mathbf{x})$ is the underlying probability density function (PDF) on $\mathcal{M}$ describing the distribution of the vertices in $\mathcal{P}$ on $\mathcal{M}$, hence $\int_{\mathcal{M}} h(\mathbf{x}) d \mathbf{x} = 1$ holds. Assume the vertices are uniformly distributed on $\mathcal{M}$, then the convergence becomes,
\begin{equation}
\underset{M \rightarrow \infty, \epsilon \rightarrow 0} {\lim} \mathbf{f}^{\top} \mathbf{L} \mathbf{f} \sim  \frac{1}{|\mathcal{M}|}\int_{\mathcal{M}} ||\nabla_{\mathcal{M}} f(\mathbf{x})||_2^2 d \mathbf{x},
\end{equation}
where $|\mathcal{M}|$ is the volume of the manifold $\mathcal{M}$.
As shown in the convergence results, as the number of samples $M$ increases, and the neighborhood size $r$ shrinks, the graph Laplacian regularization approaches the continuous limit on the right.
